Inverse molecular design and parameter optimization with H\"uckel theory using automatic differentiation

Semi-empirical quantum chemistry has recently seen a renaissance with applications in high-throughput virtual screening and machine learning. The simplest semi-empirical model still in widespread use in chemistry is H\"uckel's $\pi$-electron molecular orbital theory. In this work, we implemented a H\"uckel program using differentiable programming with the JAX framework, based on limited modifications of a pre-existing NumPy version. The auto-differentiable H\"uckel code enabled efficient gradient-based optimization of model parameters tuned for excitation energies and molecular polarizabilities, respectively, based on as few as 100 data points from density functional theory simulations. In particular, the facile computation of the polarizability, a second-order derivative, via auto-differentiation shows the potential of differentiable programming to bypass the need for numeric differentiation or derivation of analytical expressions. Finally, we employ gradient-based optimization of atom identity for inverse design of organic electronic materials with targeted orbital energy gaps and polarizabilities. Optimized structures are obtained after as little as 15 iterations, using standard gradient-based optimization algorithms.

==> extra.tex <==
Optimized $\alpha_{\ell}$
\begin{figure}[h]
    \centering
    \includegraphics[scale=0.31]{Figures/huckel_xyz_beta_c_hx_.png}
    \includegraphics[scale=0.31]{Figures/huckel_xyz_beta_exp_hx_.png}
    \includegraphics[scale=0.31]{Figures/huckel_xyz_beta_linear_hx_.png}
    \caption{The color symbols represent the optimal $\alpha_{\ell}$ parameters averaged over ten different optimization protocols with different amount training data. The initial parameters ($\blacksquare$-symbol) were taken from Ref. \cite{}.
    We considered three different parametric forms for $\beta_{\ell,k}$, (left panel) $\beta^0_{\ell,k}$,(middle panel) $\beta^{exp}_{\ell,k}$ (Eq. \ref{eqn:beta_exp}), and (right panel) $\beta^{lr}_{\ell,k}$ (Eq. \ref{eqn:beta_linear}). All parameters reported are standardized with respect to $\alpha_{C}$.}
    \label{fig:opt_alpha_N}
\end{figure}

Optimized $\beta^{0}_{\ell,k}$
\begin{figure}[h]
    \centering
    \includegraphics[scale=0.31]{Figures/huckel_h_xy_beta_c_.png}
    \includegraphics[scale=0.31]{Figures/huckel_h_xy_beta_exp_.png}
    \includegraphics[scale=0.31]{Figures/huckel_h_xy_beta_linear_.png}
    \caption{The color symbols represent the optimal $\beta^{0}_{\ell,k}$ parameters averaged over ten different optimization protocols with different amount training data. The initial parameters ($\blacksquare$-symbol) were taken from Ref. \cite{}.
    We considered three different parametric forms for $\beta_{\ell,k}$, (left panel) $\beta^0_{\ell,k}$,(middle panel) $\beta^{exp}_{\ell,k}$ (Eq. \ref{eqn:beta_exp}), and (right panel) $\beta^{lr}_{\ell,k}$ (Eq. \ref{eqn:beta_linear}). All parameters reported are standardized with respect to $\beta^0_{C,C}$.}
    \label{fig:opt_beta0_N}
\end{figure}

Optimized $R^{0}_{\ell,k}$
\begin{figure}[h]
    \centering
    \includegraphics[scale=0.33]{Figures/huckel_r_xy_beta_exp_.png}
    \includegraphics[scale=0.33]{Figures/huckel_r_xy_beta_linear_.png}
    \caption{The color symbols represent the optimal $R^{0}_{\ell,k}$ parameters averaged over ten different optimization protocols with different amount training data. The initial parameters ($\blacksquare$-symbol) were taken from Ref. \cite{}.
    We considered two different parametric forms for $\beta_{\ell,k}$, (left panel) $\beta^{exp}_{\ell,k}$ (Eq. \ref{eqn:beta_exp}), and (right panel) $\beta^{lr}_{\ell,k}$ (Eq. \ref{eqn:beta_linear}). }
    \label{fig:opt_R0_N} 
\end{figure}

Optimized $y_{\ell,k}$
\begin{figure}[h]
    \centering
    \includegraphics[scale=0.33]{Figures/huckel_y_xy_beta_exp_.png}
    \includegraphics[scale=0.33]{Figures/huckel_y_xy_beta_linear_.png}
    \caption{The color symbols represent the optimal $y_{\ell,k}$ parameters averaged over ten different optimization protocols with different amount training data. The initial value for all $y_{\ell,k}$ were set to 0.3$\AA$ \cite{AugHMO,AugHMOSSH}.
    We considered two different parametric forms for $\beta_{\ell,k}$, (left panel) $\beta^{exp}_{\ell,k}$ (Eq. \ref{eqn:beta_exp}), and (right panel) $\beta^{lr}_{\ell,k}$ (Eq. \ref{eqn:beta_linear}). }
    \label{fig:opt_y_N} 
\end{figure}
